Laplacian-guided Entropy Model in Neural Codec with Blur-dissipated Synthesis

While replacing Gaussian decoders with a conditional diffusion model enhances the perceptual quality of reconstructions in neural image compression, their lack of inductive bias for image data restricts their ability to achieve state-of-the-art perceptual levels. To address this limitation, we adopt a non-isotropic diffusion model at the decoder side. This model imposes an inductive bias aimed at distinguishing between frequency contents, thereby facilitating the generation of high-quality images. Moreover, our framework is equipped with a novel entropy model that accurately models the probability distribution of latent representation by exploiting spatio-channel correlations in latent space, while accelerating the entropy decoding step. This channel-wise entropy model leverages both local and global spatial contexts within each channel chunk. The global spatial context is built upon the Transformer, which is specifically designed for image compression tasks. The designed Transformer employs a Laplacian-shaped positional encoding, the learnable parameters of which are adaptively adjusted for each channel cluster. Our experiments demonstrate that our proposed framework yields better perceptual quality compared to cutting-edge generative-based codecs, and the proposed entropy model contributes to notable bitrate savings.

==> sec/6_Acknowlegment.tex <==
\section{Conclusion}
We developed a neural image compression model which improves perceptual image quality using a non-isotropic diffusion decoder. This decoder's inductive bias effectively separates frequency components, leading to the creation of high-quality images. Moreover, we introduce an innovative entropy model that optimizes the trade-off between compression efficiency and decoding speed. This entropy model, founded on the Transformer architecture with Laplacian-shaped positional encoding, establishes a strong global spatial context. Our results underscore the efficacy of leveraging diffusion models and advanced entropy modeling to achieve outstanding image compression performance.
